Extracting Radiological Findings With Normalized Anatomical Information Using a Span-Based BERT Relation Extraction Model

Medical imaging is critical to the diagnosis and treatment of numerous medical problems, including many forms of cancer. Medical imaging reports distill the findings and observations of radiologists, creating an unstructured textual representation of unstructured medical images. Large-scale use of this text-encoded information requires converting the unstructured text to a structured, semantic representation. We explore the extraction and normalization of anatomical information in radiology reports that is associated with radiological findings. We investigate this extraction and normalization task using a span-based relation extraction model that jointly extracts entities and relations using BERT. This work examines the factors that influence extraction and normalization performance, including the body part/organ system, frequency of occurrence, span length, and span diversity. It discusses approaches for improving performance and creating high-quality semantic representations of radiological phenomena.

==> tables/entity_perf_anatomy.tex <==








\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{l}{\textbf{Exact match}} & & \multicolumn{3}{l}{\textbf{Any overlap}} \\  \cmidrule{2-4} \cmidrule{6-8}
                       & \textbf{P} & \textbf{R}    & \textbf{F1}   & &  \textbf{P} & \textbf{R}    & \textbf{F1}  \\ \midrule
SpERT, anatomy only    &            &               &               & &             &               &     \\
SpERT                  &            &               &               & &             &               &     \\ \bottomrule
%SpERT+                 &            &               &               & &             &               &     \\ \bottomrule
\end{tabular}

==> tables/entity_perf_finding.tex <==








\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{l}{\textbf{Exact match}} & & \multicolumn{3}{l}{\textbf{Any overlap}} \\  \cmidrule{2-4} \cmidrule{6-8}
                       & \textbf{P} & \textbf{R}    & \textbf{F1}   & &  \textbf{P} & \textbf{R}    & \textbf{F1}  \\ \midrule
SpERT, anatomy only    &            &               &               & &             &               &     \\
SpERT                  &            &               &               & &             &               &     \\
SpERT+                 &            &               &               & &             &               &     \\ \bottomrule
\end{tabular}

==> tables/model_config.tex <==


\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}



\begin{tabular}{m{1.4in} M{0.8in} M{0.8in}}
\toprule
\textbf{Parameter}              & \textbf{Anatomy Normalization}  & \textbf{Relation Extraction} \\ \midrule
Pretrained BERT model           & \multicolumn{2}{c}{\textit{Bio+Clinical BERT}\cite{alsentzer-etal-2019-publicly}}  \\
Span width embedding dim.       &  25       & 25    \\
Optimizer                       &  Adam     & Adam  \\
Dropout                         &  0.05     & 0.20  \\
Max gradient norm               &  1.0      & 1.0   \\
Learning rate                   &  5e-5     & 5e-5  \\
Batch size                      &  50       & 20    \\
Epochs                          &  15       & 20    \\
Learning rate warmup            &  --       & 0.1   \\
Weight decay                    &  --       & 0.01  \\
Negative entity count           &  --       & 100   \\                                
Negative relation count         &  --       & 100   \\
Relation filter threshold       &  --       & 0.4   \\
Max span width                  &  --       & 10    \\
Maximum span pairs              &  --       & 1000  \\ \bottomrule
\end{tabular}


==> tables/relation_perf.tex <==






\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{l}{\textbf{Exact match}} & & \multicolumn{3}{l}{\textbf{Any overlap}} \\ \cmidrule{2-4} \cmidrule{6-8}
                                & \textbf{P}  & \textbf{R}  & \textbf{F1}  & & \textbf{P}  & \textbf{R}  & \textbf{F1}  \\ \midrule
SpERT                           &             &             &              & &             &             &              \\
SpERT+                          &             &             &              & &             &             &          \\ \bottomrule   
\end{tabular}

==> tables/relation_performance_SPERT_ONLY.tex <==

















%\begin{tabular}{lllllllll}
\begin{tabular}{m{1.6in} cccccccc}
\toprule
\multirow{2}{*}{\textbf{Relation}} &\multirow{2}{*}{\textbf{\# gold}} & \multicolumn{3}{c}{\textbf{Exact match}} & & \multicolumn{3}{c}{\textbf{Any overlap}} \\  \cmidrule{3-5} \cmidrule{7-9}
                            &           & \textbf{P}    & \textbf{R}    & \textbf{F1}   & & \textbf{P}  & \textbf{R}    & \textbf{F1}  \\ \midrule
Finding-Anatomy             & 1,380     & 0.64          &  0.60         & 0.62          & & 0.75        & 0.69          & 0.72      \\
Finding-Anatomy Subtype     & 1,380     & 0.60          &  0.56         & 0.58          & & 0.69        & 0.64          & 0.67      \\ \bottomrule
\end{tabular}

==> tables/span_performance_SPERT_ONLY.tex <==













%\begin{tabular}{lllllllll}
\begin{tabular}{m{1.6in} cccccccc}
\toprule
\multirow{2}{*}{\textbf{Span label}} &\multirow{2}{*}{\textbf{\# gold}} & \multicolumn{3}{c}{\textbf{Exact match}} & & \multicolumn{3}{c}{\textbf{Any overlap}} \\  \cmidrule{3-5} \cmidrule{7-9}
                    &       & \textbf{P}    & \textbf{R}    & \textbf{F1}   & & \textbf{P}  & \textbf{R}    & \textbf{F1}  \\ \midrule
Finding             & 2,122 & 0.82          & 0.83          & 0.83          & & 0.91        & 0.92          & 0.91      \\
Anatomy             & 1,153 & 0.75          & 0.68          & 0.71          & & 0.83        & 0.76          & 0.79      \\ 
Anatomy Subtype     & 1,153 & 0.70          & 0.64          & 0.67          & & 0.77        & 0.70          & 0.73    \\ \bottomrule
\end{tabular}
